BubbleNet: Inferring micro-bubble dynamics with semi-physics-informed deep learning

Micro-bubbles and bubbly flows are widely observed and applied in chemical engineering, medicine, involves deformation, rupture, and collision of bubbles, phase mixture, etc. We study bubble dynamics by setting up two numerical simulation cases: bubbly flow with a single bubble and multiple bubbles, both confined in the microchannel, with parameters corresponding to their medical backgrounds. Both the cases have their medical background applications. Multiphase flow simulation requires high computation accuracy due to possible component losses that may be caused by sparse meshing during the computation. Hence, data-driven methods can be adopted as an useful tool. Based on physics-informed neural networks (PINNs), we propose a novel deep learning framework BubbleNet, which entails three main parts: deep neural networks (DNN) with sub nets for predicting different physics fields; the semi-physics-informed part, with only the fluid continuum condition and the pressure Poisson equation $\mathcal{P}$ encoded within; the time discretized normalizer (TDN), an algorithm to normalize field data per time step before training. We apply the traditional DNN and our BubbleNet to train the coarsened simulation data and predict the physics fields of both the two bubbly flow cases. The BubbleNets are trained for both with and without $\mathcal{P}$, from which we conclude that the 'physics-informed' part can serve as inner supervision. Results indicate our framework can predict the physics fields more accurately, estimating the prediction absolute errors. Our deep learning predictions outperform traditional numerical methods computed with similar data density meshing. The proposed network can potentially be applied to many other engineering fields.

==> deleted.tex <==

\section*{Appendix. Supplementary figures}


The training error, specifically the relative error $\overline{\epsilon}$, shows how well the NN approximate the training data of the network input and supervision data, takes the form:
\[\overline{\epsilon} = {\mathcal{W}_{pred} - \mathcal{W}_{train} \over \mathcal{W}_{train}}\]
where $\mathcal{W}_{pred}$ is the NN prediction by iterations during training and $\mathcal{W}_{train}$ is the training data.


The relative errors of both the DNN and \textsf{BubbleNet} training on the physics fields $u,\ v,\ p,\ \phi$, for both the two bubbly flow cases are shown in figures and , in which the upper side views $\overline{\epsilon}$ are in larger data scale adjusting the NN with higher $\overline{\epsilon}$, and in the lower views $\overline{\epsilon}$ are in the data scale adjusting the NN with lower $\overline{\epsilon}$. From both the two figures it's hard to conclude or determine which NN structure performs better during the training since $\overline{\epsilon}$ varies from different physics fields. For the single bubble case, \textsf{BubbleNet} displays higher $\overline{\epsilon}$ on $u,\ v,$ and $\phi$ fields, indicating less approximation accuracy on the training data. For the multiple bubbles flow case, \textsf{BubbleNet} displays lower $\overline{\epsilon}$ on $p$ and $\phi$, contending more accurate training approximations. 

\begin{figure}
    \centering
    \includegraphics[scale=0.8]{images/single_rerr.pdf}
    \caption{The relative errors $\overline{\epsilon}$ for both the DNN and \textsf{BubbleNet} predicted physics field $u,\ v,\ p,\ \phi$ considering the training data, for the single bubble flow case. The blue part indicates DNN's training results and red part indicates \textsf{BubbleNet}'s training results. Note that the abscissa $\mathcal{X}$ is the normalized training data numbers (meshes). The upper sub figures indicate the relative errors adjusting the data with larger relative errors $\overline{\epsilon}$. \textbf{A.} The relative errors $\overline{\epsilon}_u$ of velocity $u$. \textbf{B.} The relative errors $\overline{\epsilon}_v$ of velocity $v$. \textbf{C.} The relative errors $\overline{\epsilon}_p$ of pressure $p$. \textbf{D.} The relative errors $\overline{\epsilon}_\phi$ of pressure $\phi$.}
    \label{rerr_single}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[scale=0.8]{images/sys_rerr.pdf}
    \caption{The relative errors $\overline{\epsilon}$ for both the DNN and \textsf{BubbleNet} predicted physics field $u,\ v,\ p,\ \phi$ considering the training data, for the multiple bubbles flow case. The blue part indicates DNN's training results and red part indicates \textsf{BubbleNet}'s training results. Note that the abscissa $\mathcal{X}$ is the normalized training data numbers (meshes). The upper sub figures indicate the relative errors adjusting the data with larger relative errors $\overline{\epsilon}$. \textbf{A.} The relative errors $\overline{\epsilon}_u$ of velocity $u$. \textbf{B.} The relative errors $\overline{\epsilon}_v$ of velocity $v$. \textbf{C.} The relative errors $\overline{\epsilon}_p$ of pressure $p$. \textbf{D.} The relative errors $\overline{\epsilon}_\phi$ of pressure $\phi$.}
    \label{rerr_multi}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.21]{images/mesh_coarse.pdf}
    \caption{The meshing of the two bubble flow cases with different mesh density. \textbf{A1.} The dense meshing of the single bubble flow case, with 24182 meshes. \textbf{A2.} The dense meshing of the multiple bubbles flow case, with 75302 meshes. Note that both \textbf{A1} and \textbf{A2} meshing are adopted for the simulation we used to obtain our NN's training data. \textbf{B1.} The coarse meshing of the single bubble flow case, with 2102 meshes. \textbf{B2.} The dense meshing of the multiple bubbles flow case, with 7833 meshes.}
    \label{comparison-of-meshing}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[scale=0.39]{images/Re.pdf}
    \caption{The Reynold's number $Re$ distribution along the space-time domian for both the two bubble flow cases. Note that $\mathcal{X}$ is the normalized coordinates of meshing elements $\mathbb{X}$, $\tau$ is the normalized time $t$. \textbf{A}. The $Re$ distribution for the single bubble flow $Re_1$. \textbf{B}. The $Re$ distribution for the multiple bubbles flow $Re_2$.}
    \label{reynolds}
\end{figure}
The Reynold's number $Re$ distribution along the space-time domain is shown in figure \ref{reynolds}. To signify the space domain, we first use $\mathbb{X} = \left[ (x_1, y_1), (x_2, y_2), ..., (x_n, y_n)\right]$ for the $n$ meshing elements, then normalize the $\mathbb{X}$ into the scale of $[0,\ 1]$. And $\tau$ is the normalized time $t$.

\begin{figure}
    \centering
    \includegraphics[scale=0.25]{images/component.pdf}
    \caption{The two-phase flow's liquid ratio ($\phi_l / \left( \phi_l + \phi_g\right)$) of the two bubble flow cases. \textbf{A}. The liquid ratio for the single bubble flow case, where the blue dots is the simulation results, and the red dotted line is the theoretical results, calculated from the area ratio. \textbf{B}. The liquid ratio for the multiple bubbles flow case, where the blue dots is the simulation results, and the red dotted line is the theoretical results.}
    \label{component}
\end{figure}

A comparison for coarsened dense meshing CFD data result (first row), traditional deep neural network predictions (second row), \textsf{BubbleNet} predictions (third row), and the coarse meshing CFD calculated results of the phase function $\phi$ (fourth row) for the two bubble flow cases. The first column indicates the single bubble flow case and the second column indicates the multiple bubbles flow case. 


\subsection{Error analysis\label{error}}

We estimate the absolute error $|\epsilon|$ of predictions for detailed comparison and estimation for different deep learning algorithms. As previously defined, $\mathcal{U}$ is the real physics computed by simulations and $\mathcal{W}$ is the training data for NN. Hence, we compute the predictions by $\mathcal{U}_{pred} = {\mathbb{N}}^{-1} \mathcal{W}_{pred}$, where $\mathbb{N}$ is the normalizer as introduced. $\mathcal{U}_{exact}$ denotes the computation benchmark ($u,\ v,\ p,\ \phi$) by simulations. The absolute errors writes:
\[|\epsilon_{\mathcal{U}}| = |\mathcal{U}_{pred} - \mathcal{U}_{exact}|\]
which are used to describe how well the NNs performs on real physics predictions. To provide a general quantitative range of such errors, we can also compute $\overline{|\epsilon_{\mathcal{U}}|} = \frac{\sum_{i=1}^m(|\epsilon_{\mathcal{U}}|)}{m}$ as the mean of the whole error field.

